Commensurators of abelian subgroups and the virtually abelian dimension of mapping class groups

Let $\mathrm{Mod}(S)$ be the mapping class group of a compact connected orientable surface $S$, possibly with punctures and boundary components, with negative Euler characteristic. We prove that for any infinite virtually abelian subgroup $H$ of $\mathrm{Mod}(S)$, there is a subgroup $H'$ commensurable with $H$ such that the commensurator of $H$ equals the normalizer of $H'$. As a consequence we give, for each $n \geq 2$, an upper bound for the geometric dimension of $\mathrm{Mod}(S)$ for the family of abelian subgroups of rank bounded by $n$. These results generalize work by Juan-Pineda--Trujillo-Negrete and Nucinkis--Petrosyan for the virtually cyclic case.

==> docs/Introduction.tex <==
\section{Introduction}
Given a group $\Gamma$, we say a collection $\calF$ of subgroups of $\Gamma$ is a \emph{family} if it is non-empty, closed under conjugation and under taking subgroups. Fix a group $\Gamma$ and a family $\calF$ of subgroups of $\Gamma$. We say that a $\Gamma$-CW-complex $X$ is a \emph{model for the classifying space} $E_{\calF}\Gamma$ if every isotropy  group of $X$ belongs to the family $\calF$ and the fixed point set $X^H$ is contractible whenever  $H$ belongs to $\calF$. It can be shown that a model for the classifying space   $E_{\calF}\Gamma$ always exists and it is unique up to $\Gamma$-homotopy equivalence. We define the \emph{$\calF$-geometric dimension} of $\Gamma$   as
$$\gd_{\calF}(\Gamma)=\min\{n\in \mathbb{N}| \text{ there is a model for } E_{\calF}\Gamma \text{ of dimension } n \}.$$
Examples of  families of subgroups are: the family that only consists of the trivial subgroup $\{1\}$, and the family $\fin$ of finite subgroups of $\Gamma$. The $\calF$-geometric dimension  has been widely studied in the last decades, and the present paper contributes to this topic.

Let $n\geq0$ be an integer. A group is said to be \emph{virtually $\mathbb{Z}^n$} if it contains a subgroup of finite index isomorphic to $\mathbb{Z}^n$. Define the family \[\calF_n=\{H\leq\Gamma| H \text{ is virtually } \mathbb{Z}^r \text{ for some 
} 0\le r \le n \}.\] The  families $\{1\}$, $\calF_0=\fin$ and $\calF_1=\vcyc$  are relevant due to its connection with the Farrell-Jones and Baum-Connes isomorphism conjectures.  The families $\calF_n$  have been recently studied by
several people, see for instance \cite{SS20}.

\tableofcontents

==> docs/Push-out_constructions_for_classifying_spaces.tex <==
\section{Preliminaries on the Mapping Class Group}

\subsection{Definition and notation}
\begin{definition}
Let $S$ be a compact surface. We define the mapping class group $\mcg(S)$ as the isotopy class of orientation  preserving difeomorphisms of $S$  that restrict to the identity on the boundary $\partial S$.
\end{definition}


\subsection{Cutting and capping homomorphisms}

\subsection{Reduction systems for abelian subgroups}



\begin{definition}
An essential curve in $S$ is a simple closed curve of $S$  that is not homotopic to a point, a puncture  or  a boundary component of $S$.   
\end{definition}

\begin{definition}(Complex of curves)
Let $S$ be  a compact, orientable surface. The complex of curves $C(S)$ is the abstract simplex that has as vertices $V(S)$ the set of essential curves, and has a $k$-simplex for each  $(k+1)$-tuple of vertices, where each pair of corresponding isotopy classes
have disjoint representants.
\end{definition}

\begin{definition}
A subgroup $H$ of $\mcg(S)$ is reducible if there  is a nonempty simplex $\sigma$ of the complex of curves $C(S)$ such that $h\sigma=\sigma$ for all $h$ in $H$. In otherwise $H$ is irreducible. We call $\sigma$ a reduction system for $H$.  \end{definition}

\textcolor{red}{Falta definir $\mcg(S)[m]$.}

\begin{definition}(Canonical reduction system of a subgroup of $\mcg(S)$)
Let $H$ be a subgroup of $\mcg(S)$ consisting of pure elements. An isotopy class $\alpha \in V(S)$ is called an essential reduction class for $H$ if the following two conditions are satisfied: \begin{enumerate}[a)]
    \item  $f(\alpha)=\alpha$ for all $f\in H$;
    \item If $\beta\in V(S)$ and $i(\alpha,\beta)\neq 0$, then $g(\beta)\neq \beta$ for some $g\in H$.
\end{enumerate} 
We denote the set of essential reduction classes for $H$ by $\sigma(H)$. We call $\sigma(H)$ a cononical reduction system for $H$. 
Let  $K$ be  an arbitrary subgroup of $\mcg(S)$  and $L$ a normal subgroup of $K$ that has finite index in $K$ and consist of pure elements. We define a canonical reduction system for $K$ as $\sigma(K)=\sigma(L)$. This definition not depend of the subgroup $L$ see \cite[Section 7.4]{Ivanov:subgroups}
\end{definition}

\textcolor{red}{Hay que mencionar que después de cortar $S$ a través del sistema canónico de reducción, hay componentes donde $H$ actúa trivialmente y otras donde actúa reduciblemente. Las acciones reducibles a su vez, pueden ser finitas o contener un elemento pseudoAnosov. Finalmente, pasando a un subgroup de índice finito de $H$, podemos suponer que la acción en las componentes es trivial o cíclica infinita generada por un pseudoAnosov.}

\begin{lemma}\label{lem:H:has:reduction:system}
 Let $m\ge 3$. Let $H$ be  a free abelian  subgroup of $\mcg(S)[m]$ of rank  at least $2$. Then $H$ is reducible and has a nonempty canonical reduction system.
\end{lemma}
\begin{proof}
Since $H$ is free-torsion group, we have by Nielsen-Thurston classification of elements of $\mcg(S)$ that every element of $H$ either reducible or pseudo-Anosov. But by\textcolor{red}{reference pending} the centralizer of a pseudo-Anosov element is virtually cyclic, since $H$ is a free abelian of rank at least 2 we have that the centralizer of any element of $H$ is not virtually cyclic.  It follow that $H$ has only reducible elements. By before and  \cite[Corollary 7.14]{Ivanov:subgroups} $H$ is reducible, now by \cite[Corollary 7.17]{Ivanov:subgroups} $H$ has a nonempty cononical reduction system  $\sigma=\{\alpha_1, \cdots, \alpha_n\}$.
\end{proof}
 


\section{Geometric dimensions for families}

\subsection{Definitions}

\subsection{Some useful tools}

\begin{proposition}\cite[Lemma 2.4]{tomasz}\label{lemma:key:1}
 Let $G$ be a countable group and $\calF$ a family of subgroups of $G$ such that any $H\in \calF$ is contained is some finitely generated subgroup of $G$. Suppose that there is an integer $d>0$ such that for every finitely generated subgroup $K$ of $G$ we have $\gd_{\calF\cap K}K\leq d$. Then $\gd_{\calF}G\leq d+1$.
 \end{proposition}
 \begin{proposition}\cite[Proposition 5.1 (i)]{LW12}\label{pro:key:2}
 Let $G$ be a group and $\calF$ and $\calG$ be two families of subgroups such that $\calF\subset \calG$. Suppose for every $H\in \calG$ we have $\gd_{\calF\cap H}H\leq d$. Then $\gd_{\calF}G\leq\gd_{\calG}G+d$.
 \end{proposition}
 
 
 
\begin{proposition}\cite[Lemma 5.7]{Nucinkis:Petrosyan}\label{vcd:s.e.s:1}
Let $1\to \Z^n\to G\to Q\to 1$ be an extension of groups where $Q$ is finitely generated with $\vcd Q = K < \infty$. Then $\vcd G = n+k$. 
\end{proposition}
 
 
  
\begin{proposition}\cite[Corollary 5.8]{Nucinkis:Petrosyan}\label{pro:key:3}
Let $1\to \Z^n\to G\to Q\to 1$ be a extension of groups where $Q$ has a cocompact model for $\underline{E}Q$ of dimension $\vcd Q =k< \infty$. Then $G$ has a cocompact model for $\underline{E}G$ of dimension $\underline{\gd}G=\vcd G=n+k$. 
\end{proposition}

\subsection{Some results on the Mapping Class Group}

 \section{Push-out constructions for classifying spaces}
 
 \subsection{The Lück and Weiermann construction}
 \textcolor{red}{Tal vez convenga enunciar directamente Luck-Weiermann para nuestro caso, es decir, con la relación de conmensuración definida en $\calF_n-\calF_{n-1}$. De esta manera $N_G[H]$ siempre denotará al conmensurador de $H$ sin ambiguedad.}
 
 \begin{definition}
 Let $\calF\subset\calG$ be two families of subgroups of $G$. Let $\sim$ be  an equivalence relation in $\calG-\calF$. We say that $\sim$ is strong  if the following it satisfied 
 
\begin{enumerate}[a)]
    \item If  $H, K \in \calG-\calF$ with $H\subseteq K$, then $H\sim K$;
    \item If $H, K \in \calG-\calF$ and $g\in G$, then $H\sim K$ if and only if $gHg^{-1} \sim gKg^{-1}$.
\end{enumerate}
 \end{definition}
 
 \textcolor{red}{Falta definir $N_G[H]$. Hay que darle una revisada a todas estas definiciones.}
 
Let $\sim$ be  a strong equivalence in $\calG-\calF$. Let $[H]$ be a class of $(\calG-\calF)/\sim$, we define $\calG[H]=\{K\subseteq N_G[H]| K\in  \calG-\calF, [K]=[H]\}\cup (\calF\cap N_G[H])$.
 \begin{theorem}\cite[Theorem 2.3]{LW12}  Let $\calF\subset\calG$ be two families of subgroups of $G$. Let $\sim$ be  a strong equivalence  in $\calG-\calF$. Let $I$ a complete representatives class of conjugation in $(\calG-\calF)/\sim$. Choose arbitrary $N_G[H]$-CW-models for $E_{\mathcal{F}\cap N_{G}[H]}N_{G}[H]$ and $E_{ \calG[H]}N_{G}[H]$, and an arbitrary model for  $E_{\mathcal{F}}G$. Consider the  following $G$-push-out 
  \[
\begin{tikzpicture}
  \matrix (m) [matrix of math nodes,row sep=3em,column sep=4em,minimum width=2em]
  {
     \displaystyle\bigsqcup_{[H]\in I} G\times_{N_{G}[H]}E_{\mathcal{F}\cap N_{G}[H]}N_{G}[H] & E_{\mathcal{F}}G \\
      \displaystyle\bigsqcup_{[H]\in I} G\times_{N_{G}[H]}E_{ \calG[H]}N_{G}[H] & X \\};
  \path[-stealth]
    (m-1-1) edge node [left] {$\displaystyle\bigsqcup_{[H]\in I}id_{G}\times_{N_G}f_{[H]}$} (m-2-1) (m-1-1.east|-m-1-2) edge  node [above] {$i$} (m-1-2)
    (m-2-1.east|-m-2-2) edge node [below] {} (m-2-2)
    (m-1-2) edge node [right] {} (m-2-2);
\end{tikzpicture}
\]
such that $f_{[H]}$ is cellular $N_{G}[H]$-map for every $[H]\in I$ and $i$ is an inclusion of $G$-CW-complexes, or such that every map $f_{[H]}$ is an inclusion of $N_{G}[H]$-CW-complexes for every $[H]\in I$ and $i$ is a cellular $G$-map. Then $X$ is a model for $E_{G}G$.
 \end{theorem}
 
 \subsection{The push-out of a union of families}
 \textcolor{red}{Falta enunciar el pushout de una unión de familias.}
 
 
 \section{Commensurators of virtually abelian subgroups}
 
 \textcolor{red}{Hablar del contexto de estos resultados. Es decir, lo que se sabe del caso cíclico infinito de los trabajos de Juan-Pineda--Trujillo y Nucinkis--Petrosyan.}
 
 The following definition is borrowed from \cite[Definition~2.8]{tomasz}.
 
 \begin{definition}(Condition C) Let $n$ be a natural number.
We say that a group $G$ satisfies condition $\mathrm{C}_n$ if for every $H\in \calF_n$, and for all $K\subset N_{G}[H]$ finitely generated, there is $H^{\prime}\in \calF_n$ with $H^{\prime}$ commensurable with $H$ such that $\langle H, K\rangle \subset N_{G}(H^{\prime})$. Whenever $G$ satisfies condition  $\mathrm{C}_n$, for all $n$, we say $G$ satisfies condition $\mathrm{C}$. 
\end{definition}


\begin{proposition}\label{condition:c} Let $S$ be a closed surface possibly with punctures.
The mapping class group $\mcg(S)$ satisfies condition $C$.
\end{proposition}

\begin{proof}
Let $H\in \calF_n$ and let $K\subset N_{G}[H]$ finitely generated, we can assume that $H$ is free abelian by replacing $H$ with a subgroup of finite index if necessary. In   \cite[Theorem 1.1.]{MR2271769} it is proved that every solvable subgroup of $\mcg(S)$ is separable, hence $H$ is separable in $\mcg(S)$. Now by \cite[Corollary 9]{MR4138929} there is a finite index subgroup $H^{\prime}$ of $H$ that is normal in $\langle H, K\rangle$. 
\end{proof}


 \begin{proposition}\label{Normalizer:commensurator:free:abelian:subgroup}
Let $m\ge 3$. Let $H$ be  a free abelian  subgroup of $\mcg(S)[m]$ of rank  at least $2$, and let be its canonical reduction system $\sigma=\{\alpha_1, \cdots, \alpha_n\}$. Then the following statements hold.

\begin{enumerate}[(a)]
    \item There is a short exact sequence 
$$1\to \Z^k \to  N_{\mcg(S)}(H)\xrightarrow[]{\rho_{\sigma}} Q\to 1$$
where $k\leq n$, $Q\subseteq \mcg(\displaystyle\bigsqcup_{i=1}^{a}S_i)\times A$, and $A$ is virtually abelian group of rank almost $l-a$ \textcolor{red}{hay que definir $l$}.

\item $N_{\mcg(S)}[H]$ is finitely generated.
\end{enumerate}
\end{proposition}

\begin{proof} We star with the proof of the item $(a)$. We claim that $N_{\mcg(S)}[H]\subseteq \mcg(S)_{\sigma}$. Let $g\in N_{\mcg(S)}[H]$, this means that $gHg^{-1}$ is commensurable with $H$. Since   the canonical reduction system of a subgroup of $\mcg(S)$ is invariant under subgroups of finite index  we have  $\sigma(H)=\sigma(gHg^{-1}\cap H)=\sigma(gHg^{-1})$. On the other hand, we have by \cite[p. 64]{Ivanov:subgroups} that  $\sigma(gHg^{-1})=g\sigma(H)$, it follows that $g\sigma(H)=\sigma(H)$, this finishes the proof of the claim.

We consider the cutting homomorphism $\rho_{\sigma}\colon \mcg(S)_{\sigma}\to \mcg(\hat{S}_{\sigma})$ that has $\ker(\rho_{\sigma})=\Z^n$. Note that $N_{\mcg(S)}(H)\subseteq N_{\mcg(S)}[H]$ then, using the claim in the previous paragraph, we can restrict $\rho_\sigma$ to obtain the following short exact sequence 
$$1\to \Z^n \cap N_{\mcg(S)}(H) \to  N_{\mcg(S)}(H)\xrightarrow[]{\rho_{\sigma}} Q\to 1$$
where $Q=\rho_{\sigma}(N_{\mcg(S)}(H))$. \textcolor{red}{Passing to a finite index subgroup if its necessary we have by \cite[Theorem 7.11]{Ivanov:subgroups} that $\rho_{\sigma}(H)|_{\mcg(S_i)}$ is trivial or irreducible (tal vez pondremos esto como hipótesis).} By re-indexing if needed we can write $\hat{S}_{\sigma}=\bigsqcup_{i=1}^{a}S_i \bigsqcup_{j=a+1}^{l}S_i$ where $\rho_{\sigma}(H)|_{\mcg(S_i)}$ is trivial for all $1\le i\le a$ and $\rho_{\sigma}(H)|_{\mcg(S_i)}$ is irreducible  for all $a+1\le i\le l$.

We claim that $N_{\mcg(\hat{S}_{\sigma})}(\rho_{\sigma}(H))\subseteq \mcg(\bigsqcup_{i=1}^{a}S_i)\times \mcg(\bigsqcup_{j=a+1}^{l}S_i)$. Suppose that this is not the case, then there exists $g\in N_{\mcg(\hat{S}_{\sigma})}(\rho_{\sigma}(H))$ that sends $S_i$ for some $1\leq i \leq a$ to $S_j$ for some $a+1\leq j \leq l$. Then for all $x\in S_i$, and for all $h\in H$, we have $\rho_{\sigma}(h)g(x)=g\rho_{\sigma}(x)=g(x)$. Therefore $\rho_{\sigma}(H)$ act trivially in $S_j$ and this is a contradiction.

Note that $\rho_{\sigma}(H)\subseteq \{ 1 \}\times  \mcg(\bigsqcup_{j=a+1}^{l}S_i)$ it follows that 
\[N_{\mcg(\hat{S}_{\sigma})}(\rho_{\sigma}(H))\subseteq \mcg(\bigsqcup_{i=1}^{a}S_i)\times N_{\mcg(\bigsqcup_{j=a+1}^{l}S_i)}(\rho_{\sigma}(H)).\] We proof that $N_{\mcg(\bigsqcup_{j=a+1}^{l}S_i)}(\rho_{\sigma}(H))$ is virtually abelian, for this is sufficient to show that $N_{\mcg(\bigsqcup_{j=a+1}^{l}S_i)^{0}}(\rho_{\sigma}(H))$ is virtually abelian. Note that we have projections $\mcg(\bigsqcup_{j=a+1}^{l}S_i)^{0}= \prod_{i=a+1}^{l}\mcg(S_i) \xrightarrow[]{\varphi_{i}} \mcg(S_i)$, we have the following diagram 

 \[
\begin{tikzpicture}
  \matrix (m) [matrix of math nodes,row sep=3em,column sep=4em,minimum width=2em]
  {
     N_{\mcg(\bigsqcup_{j=a+1}^{l}S_i)^{0}}(\rho_{\sigma}(H)) & \prod_{i=a+1}^{l}\mcg(S_i) \\
      N_{\mcg(S_i)}(\varphi_i(\rho_{\sigma}(H)))& \mcg(S_i) \\};
  \path[-stealth]
    (m-1-1) edge node [left] {} (m-2-1) (m-1-1.east|-m-1-2) edge  node [above] {$i$} (m-1-2)
    (m-2-1.east|-m-2-2) edge node [below] {$i$} (m-2-2)
    (m-1-2) edge node [right] {} (m-2-2);
\end{tikzpicture}
\]
Note that $ V_i:=N_{\mcg(S_i)}(\varphi_i(\rho_{\sigma}(H)))$ is virtually cyclic and $N_{\mcg(\bigsqcup_{j=a+1}^{l}S_i)^{0}}(\rho_{\sigma}(H)) \subseteq \prod_{i=a+1}^{l}V_i$, it follows that $N_{\mcg(\bigsqcup_{j=a+1}^{l}S_i)^{0}}(\rho_{\sigma}(H))$ is virtually abelian.\\

Now we proof item $(b)$. In the item $(a)$ we showed that $N_{\mcg(S)}[H]\subseteq \mcg(S)_{\sigma}$, then also we have a short exact sequence 
 $$1\to \Z^n \cap N_{\mcg(S)}[H] \to  N_{\mcg(S)}[H]\xrightarrow[]{\rho_{\sigma}} K\to 1$$
 where $K=\rho_{\sigma}(N_{\mcg(S)}[H])$. It is easy to proof that  $\rho_{\sigma}(N_{\mcg(S)}[H])\subseteq N_{\mcg(\hat{S}_\sigma)}([\rho_{\sigma}(H)])$.  Using the same decomposition of  $\hat{S}_{\sigma}=\bigsqcup_{i=1}^{a}S_i \bigsqcup_{j=a+1}^{l}S_i$ as in the item $(a)$ we can proof that $N_{\mcg(\hat{S}_\sigma)}([\rho_{\sigma}(H)])\subseteq \mcg(\bigsqcup_{i=1}^{a}S_i)\times \mcg(\bigsqcup_{j=a+1}^{l}S_i)$, since $\rho_{\sigma}(H)\subseteq \mcg(\bigsqcup_{j=a+1}^{l}S_i)$  it follows that  $N_{\mcg(\hat{S}_\sigma)}([\rho_{\sigma}(H)])=\mcg(\bigsqcup_{i=1}^{a}S_i)\times N_{\mcg(\bigsqcup_{j=a+1}^{l}S_i)}[\rho_{\sigma}(H)]$. The little variation of the  argument  given in the item $(a)$ show that  $N_{\mcg(\bigsqcup_{j=a+1}^{l}S_i)}[\rho_{\sigma}(H)]$ is virtually abelian. Hence $N_{\mcg(\hat{S}_\sigma)}([\rho_{\sigma}(H)])=\mcg(\bigsqcup_{i=1}^{a}S_i)\times N_{\mcg(\bigsqcup_{j=a+1}^{l}S_i)}[\rho_{\sigma}(H)]$ is finite generated.
 \end{proof}
 
 \begin{proposition}\label{norrmalizer:commensurator:equal}
Let $S$ be a connected, closed, oriented  and possibly with a finite number of punctures. Let $H$ be  a free abelian  subgroup of $\mcg(S)$ of rank $k\ge 2$. Then there is a subgroup $L\leq H$ of finite index such that $N_{\mcg(S)}[L]=N_{\mcg(S)}(L)$.
\end{proposition}
\begin{proof}
  By \cref{Normalizer:commensurator:free:abelian:subgroup} $N_{\mcg(S)}[H]$ is finite generated, then by \cref{condition:c} there is a subgroup $L\leq H$ of finite index such that $\langle H, N_{\mcg(S)}[H] \rangle\subseteq N_{\mcg(S)}(L)$, but $\langle H, N_{\mcg(S)}[H] \rangle=N_{\mcg(S)}[H]= N_{\mcg(S)}[L]$, hence $N_{\mcg(S)}[L]\subseteq N_{\mcg(S)}(L)$. The another contention $N_{\mcg(S)}(L) \subseteq N_{\mcg(S)}[L]$ is always true, this finish the proof. 
\end{proof}

 

==> docs/virtually_abelian_dimension_of_mcg_.tex <==
\section{Vitually abelian dimension of MCG}



\begin{theorem}
Let $S$ be a connected, closed, oriented  and possibly with a finite number of punctures. Denoted by $G=\mcg(S)$. Then $\gd_{\calF_2}(G)\leq \gd_{\calF_1}(G)+1$.
\end{theorem}
\begin{proof}
 Let $\sim$ be  the equivalence relation in $\calF_2-\calF_1$ defined by commensurability. Let $I$ be  a set complete of representatives of the conjugacy classes in  $\calF_2-\calF_1/\sim$. Then by \cite[Theorem 2.3]{LW12} the following homotopy  $G$-push-out give a model of $E_{\calF_2}G$
 
   \[
\begin{tikzpicture}
  \matrix (m) [matrix of math nodes,row sep=3em,column sep=4em,minimum width=2em]
  {
     \displaystyle\bigsqcup_{[H]\in I} G\times_{N_{G}[H]}E_{\calF_1}N_{G}[H] & E_{\calF_1}G \\
      \displaystyle\bigsqcup_{[H]\in I} G\times_{N_{G}[H]}E_{ \calF_2[H]}N_{G}[H] & X \\};
  \path[-stealth]
    (m-1-1) edge node [left] {$\displaystyle\bigsqcup_{[H]\in I}id_{G}\times_{N_G}f_{[H]}$} (m-2-1) (m-1-1.east|-m-1-2) edge  node [above] {$i$} (m-1-2)
    (m-2-1.east|-m-2-2) edge node [below] {} (m-2-2)
    (m-1-2) edge node [right] {} (m-2-2);
\end{tikzpicture}
\]
the dimension of $X$ is bound by the $\max \{\gd_{\calF_1}(N_{G}[H])+1, \gd_{\calF_1}(G), \gd_{\calF_2[H]}(N_{G}[H])\}_{H\in I}$. Then 
\begin{equation} \label{eq1}
\begin{split}
\gd_{\calF_2}(G) & \leq \max \{\gd_{\calF_1}(N_{G}[H])+1, \gd_{\calF_1}(G), \gd_{\calF_2[H]}(N_{G}[H])\}_{H\in I} \\
 & \leq \max \{ \gd_{\calF_1}(G)+1, \gd_{\calF_2[H]}(N_{G}[H])\}_{H\in I}
\end{split}
\end{equation}
the second inequality it follows from $\gd_{\calF_1}(N_{G}[H])\leq \gd_{\calF_1}(G)$. Now we give a bound of $\gd_{\calF_2[H]}(N_{G}[H])$. By \cref{norrmalizer:commensurator:equal} there is a subgroup $L\leq H$ of finite index  such that $N_{G}[L]=N_{G}(L)$, then we can replace $N_{G}[H]$ by $N_{G}[L]=N_{G}(L)$. The family $$\calF_2[L]=\{K\subseteq N_G[L]| K\in  \calF_2-\calF_1, [K]=[L]\}\cup (\calF_1\cap N_G[L])$$ can be write as the union of two families $\calF_2[L]=\calG \cup \calF$ where $\calG$ is the family generated by  $\{K\subseteq N_G[L]| K\in  \calF_2-\calF_1, [K]=[L]\}$ union the family $\calF_0$ of $N_G[L]$, and $\calF$ is family $(\calF_1\cap N_G[L])$. By \cite[Lemma 4.4]{MR2832565} the following homotopy  $N_G(L)$-push-out give a model for $E_{\calF_2[L]}N_G(L)$

  \[
\begin{tikzpicture}
  \matrix (m) [matrix of math nodes,row sep=3em,column sep=4em,minimum width=2em]
  {
     E_{\calF \cap \calG}N_{G}(L) & E_{\calF}N_{G}(L) \\
      E_{\calG}N_{G}(L) & Y \\};
  \path[-stealth]
    (m-1-1) edge node [left] {} (m-2-1) (m-1-1.east|-m-1-2) edge  node [above] {} (m-1-2)
    (m-2-1.east|-m-2-2) edge node [below] {} (m-2-2)
    (m-1-2) edge node [right] {} (m-2-2);
\end{tikzpicture}
\]

Note that   $\dim(Y) \leq\max \{\gd_{\calF}(N_{G}(L)), \gd_{\calF \cap \calG}(N_{G}(L)), \gd_{\calG}(N_{G}(L))\}$. Then 
\begin{equation} \label{eq2}
\begin{split}
\gd_{\calF_2[L]}(N_{G}[L]) & \leq\max \{\gd_{\calF}(N_{G}(L)), \gd_{\calF \cap \calG}(N_{G}(L)), \gd_{\calG}(N_{G}(L))\} \\
 & \leq \max \{ \gd_{\calF_1}(G), \gd_{\calF \cap \calG}(N_{G}(L)), \gd_{\calG}(N_{G}(L))\}.
\end{split}
\end{equation}
Now we prove the followings inequalities
\begin{enumerate}[i)]
    \item $\gd_{\calG}(N_{G}(L))\leq \vcd W(L)$.
    \item $\gd_{\calF \cap \calG}(N_{G}(L)) \leq \vcd W(L)+3$
\end{enumerate}
 First we going to show $\gd_{\calG}(N_{G}(L))\leq \vcd W(L)$. A model for $E_{\calF_0}W(L)$ is a model for $E_{\calG}N_{G}(L)$ via the action given by the projection $N_{G}(L)\to N_{G}(L)/L$. 

By \cref{Normalizer:commensurator:free:abelian:subgroup} we have the following   short exact sequence 

\begin{equation}\label{s.e.s:normalaizer:1}
1\to \Z^n \cap N_{\mcg(S)}(L) \to  N_{\mcg(S)}(L)\xrightarrow[]{\rho_{\sigma}} Q\to 1\end{equation}
with $Q\subseteq \mcg(\displaystyle\bigsqcup_{i=1}^{a}S_i)\times A$ where $A$ is virtually abelian group of rank almost $l-a$. From \cref{s.e.s:normalaizer:1} we have the next short exact sequence 

\begin{equation}\label{s.e.s:weil:1}
1\to  (\Z^n \cap N_{G}(L))/(L\cap(\Z^n \cap N_{G}(L))) \to  W(L)\xrightarrow[]{\rho_{\sigma}} Q/\rho_{\sigma}(L)\to 1\end{equation}

We proof that $W(L)$ has a model for  $E_{\calF_0}W(L)$  of dimension $\vcd(W(L))$, by \cref{pro:key:3} it is enough to show that   $Q/\rho_{\sigma}(L)$ has a model for $E_{\calF_0}Q/\rho_{\sigma}(L)$ of dimension $\vcd Q/\rho_{\sigma}(L)$. Now note that   $Q/\rho_{\sigma}(L)= \mcg(\bigsqcup_{i=1}^{a}S_i)\times A/\rho_{\sigma}(L)$ then $\gd_{\calF_0}(Q/\rho_{\sigma}(L))= \gd_{\calF_0}(\mcg(\bigsqcup_{i=1}^{a}S_i))+ \gd_{\calF_0}A/\rho_{\sigma}(L)$, by \cite[Proposition 5.3]{Nucinkis:Petrosyan} we have that $\gd_{\calF_0}(\mcg(\bigsqcup_{i=1}^{a}S_i))=\vcd \mcg(\bigsqcup_{i=1}^{a}S_i)$ then by \cref{vcd:s.e.s:1} we have $\gd_{\calF_0}(Q/\rho_{\sigma}(L))= \vcd  Q/\rho_{\sigma}(L)$ as desired.


Now we bound $\gd_{\calF \cap \calG}(N_{G}[H])$. Note that $\calF \cap \calG \subset \calG$, then  by   \cref{pro:key:2} we need to find a integer $d>0$ such that for any $S\in \calG$ we have $\gd_{\calF\cap \calG\cap 
S}S\leq d$. Let $S\in \calG$ then we have three cases (i) $S$ is finite , (ii) $S$ is virtually $\Z$ or (iii) $S$ is virtually $\Z^2$. 

In the case (i) and (ii) we have $\gd_{\calF\cap \calG\cap 
S}S= 0$ since $S$ is virtually cyclic  then $S\in \calF$ but also $S\in \calG$, it follows that $S\in \calF\cap \calG\cap 
S$. In the case (iii) we have $\gd_{\calF\cap \calG\cap 
S}S= 3$ this because we going to proof that  $\calF\cap \calG\cap 
S$ is the family of virtually cyclic subgroups $\calH$ of $S$. The contention $\calF\cap \calG\cap S \subset \calH$ is clear. Remains to show that $\calH \subset \calF\cap \calG\cap S$. The fact that $S\in \calG$ and $S$ is virtually $\Z^{2}$ implies that $S$ is commensurable with $H$, then we have $N_{G}[S]=N_{G}[H]$. Let $L\in \calH$ by the before we have $L\in \calF$,  by hypothesis $S\in \calG$ and $\calG$ is a family implies also that $L\in \calG$. It follows that $L\in \calF\cap \calG\cap S$.  
Therefore we have by \cref{pro:key:2} that $\gd_{\calF \cap \calG}(N_{G}[H])\leq \vcd W(L)+3$.

Thus, by \cref{eq2} we have 
\begin{equation} \label{eq3}
\begin{split}
\gd_{\calF_2[H]}(N_{G}[H]) &=\gd_{\calF_2[L]}(N_{G}[L]) \\ 
 & \leq \max \{ \gd_{\calF_1}(G), \gd_{\calF \cap \calG}(N_{G}(L)), \gd_{\calG}(N_{G}(L))\}\\
 & \leq \max \{ \gd_{\calF_1}(G), \vcd W(L)+3, \vcd W(L)\}\\
 &= \max \{ \gd_{\calF_1}(G), \vcd W(L)+3\}\\
 &= \max \{ \gd_{\calF_1}(G), \vcd N_{G}(L)+1\}\\
 &\leq \max \{ \gd_{\calF_1}(G), \vcd G+1\}\\
&=  \gd_{\calF_1}(G).
\end{split}
\end{equation}

Finally by \cref{eq1} we have $\gd_{\calF_2}(G)\leq \gd_{\calF_1}(G)+1$.


\end{proof}
